Measuring Sound Symbolism in Audio-visual Models

Audio-visual pre-trained models have gained substantial attention recently and demonstrated superior performance on various audio-visual tasks. This study investigates whether pre-trained audio-visual models demonstrate non-arbitrary associations between sounds and visual representations$\unicode{x2013}$known as sound symbolism$\unicode{x2013}$which is also observed in humans. We developed a specialized dataset with synthesized images and audio samples and assessed these models using a non-parametric approach in a zero-shot setting. Our findings reveal a significant correlation between the models' outputs and established patterns of sound symbolism, particularly in models trained on speech data. These results suggest that such models can capture sound-meaning connections akin to human language processing, providing insights into both cognitive architectures and machine learning strategies.

==> figs/visualization_images.tex <==
\begin{figure*}[t]
  \includegraphics[width=\linewidth,trim={0 0cm 0 8cm},clip]{figs/image_only.pdf}
  \caption {Pseudowords along with the generated images.}
  \label{fig:qualitative_image}
\end{figure*}

==> figs/visualization_phonemes.tex <==
\begin{figure*}[t]
  \includegraphics[width=\linewidth,trim={0 4.5cm 0 0},clip]{figs/phoneme_only.pdf}
  \caption {Qualitative results of geometric scores using SpeechCLIP and comparision with human evaluation. \david{Several things: ``Constants'' should be ``consonants''. Second, if we are keeping this figure I suggest making it much smaller. Finally, I don't really understand what the figure is trying to convey. Are the phones organized left/right based on their affinity with pointy or round objects? If that's the case, please make it clear in the caption. Also, rather than just ranking them in order I think you should treat each axis as a real line, and place the phones along the axis at a location that is proportional to their similarity/dissimilarity to the pointy/round object}}
  \label{fig:qualitative_phoneme}
\end{figure*}

==> figs/visualizeByPhoneme.tex <==
\begin{figure*}[t]
  \includegraphics[width=\linewidth]{figs/visualize_phoneme_1.pdf}
  \caption {Qualitative results of geometric scores using SpeechCLIP and comparision with human evaluation.}
  \label{fig:qualitative}
\end{figure*}
